Confidence Estimation for Error Detection in Text-to-SQL Systems

Text-to-SQL enables users to interact with databases through natural language, simplifying the retrieval and synthesis of information. Despite the success of large language models (LLMs) in converting natural language questions into SQL queries, their broader adoption is limited by two main challenges: achieving robust generalization across diverse queries and ensuring interpretative confidence in their predictions. To tackle these issues, our research investigates the integration of selective classifiers into Text-to-SQL systems. We analyse the trade-off between coverage and risk using entropy based confidence estimation with selective classifiers and assess its impact on the overall performance of Text-to-SQL models. Additionally, we explore the models' initial calibration and improve it with calibration techniques for better model alignment between confidence and accuracy. Our experimental results show that encoder-decoder T5 is better calibrated than in-context-learning GPT 4 and decoder-only Llama 3, thus the designated external entropy-based selective classifier has better performance. The study also reveal that, in terms of error detection, selective classifier with a higher probability detects errors associated with irrelevant questions rather than incorrect query generations.

==> parts/app_tradeoff.tex <==
\section{Trade-Off between Generalization and Calibration} \label{sec:scatter}

Summing up the results from Sec. \ref{sec:cs1} and Sec. \ref{sec:cs2} we can plot the trade-off between calibration characteristic and execution match of explored models. Fig. \ref{fig:tradeoff} demonstrates the trade-off for 4 Text-to-SQL (T5-large, T5-3B, Llama 3 in SFT and LoRa setting). We use the Brier score as the measure of calibration level. Overall, we see that T5 models are much better calibrated than Llama 3 in all splits albeit not always with the highest execution match (PAUQ XSP, TSL SSP). Moreover, in the EHRSQL split we see that T5 models significantly outperform Llama 3 in both axes.

\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.95\textwidth]{images/exec_match_to_calibration_error.png}
% \vspace{-0.2cm}
    \caption{Trade-off plots between execution match and calibration for selected Text-to-SQL models (T5-large, T5-3B, Llama 3 in SFT and LoRa setting).}
    \label{fig:tradeoff}
\end{figure*}

==> parts/data.tex <==
\section{Data and Models}

For confidence estimation we use $5$ common \task models - encoder-decoder T5((\textbf{Llama3-8B SFT}) and \textbf{T5-3B}), ChatGPT based (\textbf{DAIL-SQL}) and Llama 3 8B Instruct version with LoRA fine-tuning (\textbf{Llama3-8B LoRA}) and with full instruction fine-tuning (\textbf{Llama3-8B SFT}).

For evaluated datasets, we use two \task datasets - PAUQ and EHRSQL datasets
PAUQ dataset is a refinement of a widely recognized non-synthetic benchmark SPIDER \cite{spider} for the Text-to-SQL task. This dataset presents challenges related to schema linking and the modeling of complex SQL syntax. PAUQ includes the insertion of missing values, error corrections, and the addition of new samples for poorly represented types. In particular, for those SQL queries that return None or empty list, corresponding values were added to the original databases; databases that were empty were filled with values. PAUQ contains 8{,}800 and 1{,}076 English samples for training and testing, respectively.
To sum up, PAUQ enhances the original SPIDER dataset as follows:
\begin{itemize}
\item 8 times less of empty output 
($1665 \rightarrow 231$)
\item 4 times less zero return of queries with aggregations (e.g., \textit{maximal}, \textit{minimal}) ($379 \rightarrow 85$)
\item no queries with syntax errors ($3 \rightarrow 0$)
\end{itemize}
These improvements in PAUQ are crucial for evaluating Text-to-SQL methods. They address scenarios where a model can generate a syntactically correct SQL query but fails to align with the query or return the expected values. Such queries may result in empty output, which can be mistakenly considered correct by execution match metrics. We decided to utilize that dataset because it crucial for evaluating error detection.

EHRSQL is a clinical NLP \task dataset that consists of $5124$ training samples and $1167$ testing samples of hospital worker's requests for such solution. This benchmark consists of pairs of input utterances and expected SQL queries, including cases where generating an SQL query is impossible for a given question. This dataset is linked to two open-source EHR databases—MIMIC-III \cite{johnson2016mimic} and eICU \cite{pollard2018eicu}. This benchmark includes questions that address the actual needs of a hospital and incorporate various time expressions crucial to daily healthcare work.

For evaluation, we evaluate $4$ different splits, to research uncertainty estimation behavior under different distribution shifts. The splits are the following:
\begin{itemize}
    \item \textbf{PAUQ in cross-database setting} - the original SPIDER dataset split, where the data is spitted in between train and test without database understanding. During training the model must learn to generalize to understanding novel database structures. We refer to that split as \textbf{PAUQ XSP}.
    \item \textbf{PAUQ with template shift in single database setting} - the compositional split of PAUQ dataset based on template in single database setting inspired \cite{finegan-dollak-etal-2018-improving}. Such split forces the model to demonstrate its \textit{systematicity} ability - the ability to recombine known syntax SQL elements to form novel SQL structures. We refer to that split as \textbf{Template SSP}.
    \item \textbf{PAUQ with target length shift single database setting} - another compositional split of PAUQ dataset based on length in single database setting. We put shorter samples in the training dataset, and longer samples in the test, while keeping all test tokens to appear at least once in the training dataset. We refer to that split as \textbf{TSL SSP} and such split forces the model to demonstrate its productivity ability - generate novel SQL queries that are longer than it was trained on.
    \item \textbf{EHRSQL with unanswerable questions} - is original EHRSQL split. It is main distinctive property is the presence of specific unanswerable questions. Such questions can not be answered with underlying database content or require external knowledge. Since the model is trained only \task{} pairs, such samples produce a covariate shift.
\end{itemize}

PAUQ XSP, Template SSP and TSL SSP are datasets which are fully shifted in terms of database and structures ($p(x_{tst}) \neq p(x_{tr}) \: \text{and} \: p(y_{tst}|x_{tst}) \neq p(y_{tr}|x_{tr})$). EHRSQL on the other hand is more a covariate split because all question templates are shared between splits, but in test, there are unanswerable questions present ($p(x_{tst}) != p(x_{tr})$)

==> tables/avg_error_detection_method_comparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}llll@{}}
\toprule
                          & $\mu$ Found Errors & $\mu$ Trafic lost & $\mu$ Result EX \\ \midrule
\textbf{Gaussian Mixture} & 0.62               & 0.16              & 0.45            \\
Logistic Regression       & 0.42               & 0.08              & 0.54            \\
Threshold                 & 0.64               & 0.29              & 0.28            \\ \bottomrule
\end{tabular}%
}
\caption{All error detection method comparison}
\label{tab:all_ed_method_comparison}
\end{table}

==> tables/decision_methods_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\begin{tabular}{|r|r|r|r|r|r|}
\hline
\textbf{} & \textbf{Method} & \textbf{PAUQ XSP} & \textbf{Template SSP} & \textbf{TSL SSP} & \multicolumn{1}{l|}{\textbf{EHRSQL}} \\ \hline
\multirow{3}{*}{\textbf{t5-large}} & \textbf{LR} & 0.64±0.02 & 0.46±0.02 & 0.86±0.01 & 0.78±0.02 \\ \cline{2-6} 
                                   & \textbf{GM} & 0.66±0.01 & 0.61±0.01 & 0.78±0.03 & 0.77±0.08 \\ \cline{2-6} 
                                   & \textbf{TR} & 0.03±0.01 & 0.05±0.02 & 0.02±0.02 & 0.05±0.04 \\ \hline
\multirow{3}{*}{\textbf{t5-3b}}    & \textbf{LR} & 0.56±0.03 & 0.32±0.03 & 0.84±0.01 & 0.82±0.02 \\ \cline{2-6} 
                                   & \textbf{GM} & 0.6±0.02  & 0.55±0.03 & 0.8±0.01  & 0.81±0.03 \\ \cline{2-6} 
                                   & \textbf{TR} & 0.03±0.01 & 0.06±0.05 & 0.02±0.01 & 0.05±0.01 \\ \hline
\multirow{3}{*}{\textbf{dailsql}}  & \textbf{LR} & 0.08±0.0  & 0.1±0.0   & 0.15±0.0  & 0.7±0.0   \\ \cline{2-6} 
                                   & \textbf{GM} & 0.49±0.0  & 0.34±0.0  & 0.41±0.0  & 0.78±0.0  \\ \cline{2-6} 
                                   & \textbf{TR} & 0.01±0.0  & 0.12±0.0  & 0.03±0.0  & 0.02±0.0  \\ \hline
\multirow{3}{*}{\textbf{llama3}}   & \textbf{LR} & 0.0±0.0   & 0.08±0.0  & 0.82±0.01 & 0.47±0.01 \\ \cline{2-6} 
                                   & \textbf{GM} & 0.43±0.0  & 0.08±0.0  & 0.08±0.0  & 0.42±0.02 \\ \cline{2-6} 
                                   & \textbf{TR} & 0.01±0.0  & 0.04±0.03 & 0.01±0.0  & 0.02±0.02 \\ \hline
\end{tabular}
\caption{Methods results}
\label{tab:methods results}
\end{table*}

==> tables/models_to_methods_metrics.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}cccccc@{}}
\toprule
\textbf{}                  & \textbf{}           & recall        & precision     & F1            & $\sigma$ F1 \\ \midrule
\multirow{3}{*}{T5-large}  & Logistic Regression & 0.74          & \textbf{0.67} & \textbf{0.69} & 0.01        \\ \cmidrule(l){2-6} 
                           & Gaussian Mixture    & 0.73          & 0.68          & 0.68          & 0.03        \\ \cmidrule(l){2-6} 
                           & Threshold           & \textbf{0.96} & 0.02          & 0.04          & 0.01        \\ \midrule
\multirow{3}{*}{T5-3B}     & Logistic Regression & \textbf{0.70} & 0.57          & 0.60          & 0.01        \\ \cmidrule(l){2-6} 
                           & Gaussian Mixture    & 0.64          & \textbf{0.76} & \textbf{0.67} & 0.02        \\ \cmidrule(l){2-6} 
                           & Threshold           & \textbf{0.97} & 0.02          & 0.04          & 0.02        \\ \midrule
\multirow{3}{*}{DIAL-SQL}  & Logistic Regression & \textbf{0.76} & 0.27          & 0.32          & $\le$ 0.01  \\ \cmidrule(l){2-6} 
                           & Gaussian Mixture    & 0.55          & \textbf{0.51} & \textbf{0.42} & $\le$ 0.01  \\ \cmidrule(l){2-6} 
                           & Threshold           & \textbf{0.90} & 0.02          & 0.04          & $\le$ 0.01  \\ \midrule
\multirow{3}{*}{Llama3-8B} & Logistic Regression & 0.62          & 0.40          & 0.39          & 0.02        \\ \cmidrule(l){2-6} 
                           & Gaussian Mixture    & \textbf{0.64} & \textbf{0.55} & \textbf{0.46} & 0.03        \\ \cmidrule(l){2-6} 
                           & Threshold           & \textbf{0.64} & 0.01          & 0.02          & 0.02        \\ \bottomrule
\end{tabular}%
}
\caption{Metrics of the models to metrics }
\label{tab:models_to_metrics_table}
\end{table}

==> tables/per_split_avg_scores.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}rrccc@{}}
\toprule
\textbf{}                           & \textbf{}           & Recall        & Precision     & $\sigma$   \\ \midrule
\multirow{3}{*}{PAUQ XSP}           & Logistic Regression & \textbf{0.49} & 0.28          & 0.01       \\
                                    & Gaussian Mixture    & 0.44          & \textbf{0.79} & 0.02       \\
                                    & Threshold           & 0.36          & 0.70          & 0.01       \\ \midrule
\multirow{3}{*}{Template SSP split} & Logistic Regression & \textbf{0.77} & 0.13          & 0.05       \\
                                    & Gaussian Mixture    & 0.66          & 0.29          & 0.01       \\
                                    & Threshold           & 0.25          & \textbf{0.75} & 0.01       \\ \midrule
\multirow{3}{*}{TSL SSP split}      & Logistic Regression & 0.71          & 0.77          & 0.01       \\
                                    & Gaussian Mixture    & \textbf{0.73} & 0.67          & 0.02       \\
                                    & Threshold           & 0.66          & \textbf{0.78} & 0.01       \\ \midrule
\multirow{3}{*}{EHRSQL}             & Logistic Regression & 0.67          & 0.50          & $\le$ 0.01 \\
                                    & Gaussian Mixture    & \textbf{0.76} & \textbf{0.72} & 0.02       \\
                                    & Threshold           & 0.70          & 0.34          & 0.04       \\ \bottomrule
\end{tabular}%
}
\caption{Per split method score}
\label{tab:per_split_method_score}
\end{table}

==> tables/result_metrics.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|rrrrrrrrrrrrr}
\multicolumn{1}{r|}{\textbf{Model}} &
  \multicolumn{1}{r|}{\textbf{}} &
  \multicolumn{3}{c|}{\textbf{PAUQ XSP}} &
  \multicolumn{3}{c|}{\textbf{Template SSP}} &
  \multicolumn{3}{c|}{\textbf{TSL SSP}} &
  \multicolumn{3}{c}{\textbf{EHRSQL}} \\ \cline{3-14} 
\multicolumn{1}{r|}{\textbf{}} &
  \multicolumn{1}{r|}{\textbf{}} &
  \multicolumn{1}{c}{\textbf{Acc@0}} &
  \multicolumn{1}{c}{\textbf{Acc@5}} &
  \multicolumn{1}{c}{\textbf{Acc@10}} &
  \multicolumn{1}{c}{\textbf{Acc@0}} &
  \multicolumn{1}{c}{\textbf{Acc@5}} &
  \multicolumn{1}{c}{\textbf{Acc@10}} &
  \multicolumn{1}{c}{\textbf{Acc@0}} &
  \multicolumn{1}{c}{\textbf{Acc@5}} &
  \multicolumn{1}{c}{\textbf{Acc@10}} &
  \multicolumn{1}{c}{\textbf{Acc@0}} &
  \multicolumn{1}{c}{\textbf{Acc@5}} &
  \multicolumn{1}{c|}{\textbf{Acc@10}} \\ \hline
\multirow{2}{*}{\textbf{t5-large}} &
  With CE &
  0.3±0.0 &
  0.2±0.03 &
  0.1±0.06 &
  0.42±0.03 &
  0.13±0.01 &
  -0.16±0.02 &
  0.12±0.01 &
  -0.82±0.26 &
  -1.76±0.52 &
  0.56±0.11 &
  0.35±0.02 &
  0.14±0.07 \\
 &
  No CE &
  0.63±0.01 &
  -1.2±0.03 &
  -3.03±0.06 &
  0.69±0.01 &
  -0.86±0.06 &
  -2.41±0.11 &
  0.24±0.01 &
  -3.54±0.06 &
  -7.32±0.12 &
  0.69±0.0 &
  -0.88±0.01 &
  -2.44±0.02 \\ \hline
\multirow{2}{*}{\textbf{t5-3b}} &
  With CE &
  0.39±0.03 &
  0.23±0.02 &
  0.07±0.04 &
  0.5±0.03 &
  0.15±0.01 &
  -0.2±0.02 &
  0.13±0.01 &
  -0.57±0.09 &
  -1.28±0.17 &
  0.61±0.02 &
  0.5±0.04 &
  0.39±0.06 \\
 &
  No CE &
  0.71±0.01 &
  -0.74±0.03 &
  -2.2±0.06 &
  0.74±0.02 &
  -0.57±0.12 &
  -1.88±0.21 &
  0.28±0.01 &
  -3.31±0.05 &
  -6.9±0.1 &
  0.71±0.0 &
  -0.73±0.01 &
  -2.17±0.02 \\ \hline
\multirow{2}{*}{\textbf{DAIL-SQL}} &
  With CE &
  0.53±0.0 &
  0.13±0.0 &
  -0.27±0.0 &
  0.69±0.0 &
  0.31±0.0 &
  -0.07±0.0 &
  0.55±0.0 &
  -0.55±0.0 &
  -1.65±0.0 &
  0.43±0.0 &
  -0.04±0.0 &
  -0.52±0.0 \\
 &
  No CE &
  0.77±0.0 &
  -0.41±0.0 &
  -1.58±0.0 &
  0.86±0.0 &
  0.16±0.0 &
  -0.54±0.0 &
  0.66±0.0 &
  -1.02±0.0 &
  -2.7±0.0 &
  0.54±0.0 &
  -1.75±0.0 &
  -4.04±0.0 \\ \hline
\multirow{2}{*}{\textbf{Llama 3}} &
  With CE &
  0.0±0.0 &
  0.0±0.0 &
  0.0±0.0 &
  0.68±0.0 &
  -0.88±0.03 &
  -2.43±0.05 &
  0.3±0.02 &
  -3.07±0.11 &
  -6.44±0.19 &
  0.48±0.01 &
  -1.04±0.0 &
  -2.56±0.0 \\
 &
  No CE &
  0.72±0.0 &
  -0.67±0.02 &
  -2.06±0.04 &
  0.68±0.0 &
  -0.94±0.03 &
  -2.57±0.05 &
  0.3±0.02 &
  -3.21±0.11 &
  -6.71±0.19 &
  0.56±0.01 &
  -1.65±0.05 &
  -3.86±0.09 \\ \hline
\end{tabular}%
}
\caption{Result metrics}
\label{tab:result_metrics}
\end{table*}
